A Survey on Password Guessing

Text password has served as the most popular method for user authentication so far, and is not likely to be totally replaced in foreseeable future. Password authentication offers several desirable properties (e.g., low-cost, highly available, easy-to-implement, reusable). However, it suffers from a critical security issue mainly caused by the inability to memorize complicated strings of humans. Users tend to choose easy-to-remember passwords which are not uniformly distributed in the key space. Thus, user-selected passwords are susceptible to guessing attacks. In order to encourage and support users to use strong passwords, it is necessary to simulate automated password guessing methods to determine the passwords' strength and identify weak passwords. A large number of password guessing models have been proposed in the literature. However, little attention was paid to the task of providing a systematic survey which is necessary to review the state-of-the-art approaches, identify gaps, and avoid duplicate studies. Motivated by that, we conduct a comprehensive survey on all password guessing studies presented in the literature from 1979 to 2022. We propose a generic methodology map to present an overview of existing methods. Then, we explain each representative approach in detail. The experimental procedures and available datasets used to evaluate password guessing models are summarized, and the reported performances of representative studies are compared. Finally, the current limitations and the open problems as future research directions are discussed. We believe that this survey is helpful to both experts and newcomers who are interested in password security

==> background.tex <==
\section{<<Background>>}
\cm{This section notes some ideas/comment/opinions may come out during this survey, and could be deleted in the final step}

\subsection{Special Term}
proactive password checking

rate-limiting policies

password guessability

\subsection{Important Note/Opinion}

==> metering.tex <==
\section{Password metering}
\cite{egelman2013does} analyze the impact of password metering on user behavior

\cite{carnavalet2015large} analyze password meters deployed in selected popular websites and password managers Google, Tencent QQ, Yahoo!, Twitter, eBay, Yandex, Apple, PayPal, Microsoft (three versions), Dropbox, Skype, FedEx, China railway customer service center, Drupal, LastPass, KeePass, 1Password (AgileBits, three versions) and RoboForm (Siber Systems)


password strength is not a universal value. Rather, it is highly dependent on the context in which the password is used. 
%
That is, the exact same password can have a significantly different strength depending on the application where it is utilized. 
%
For example, a Hungarian word used to login to a computer in a Spanish-based company can be a quite strong password. 
%
However, that same password, used in a Hungarian-based context would most likely be regarded as weak. 
%


A similar argument can be made for a five character password used to access remotely an account protected by a three-attempt limit (strong), compared to that same password used to access a local service with unlimited number of attempts (weak).


\subsection{Requirement/Challenge}
The set of requirements for password metering \cite{golla2018accuracy}

Storage (especially running in client side (mobile devices))

Running time (response time)

Should be able to capture both the "low entropy words", and "leaked passwords", as well as "common pattern"


Impact of meter to the password \cite{ur2012does}, survey the popular password metering websites

Impact of password-composition policy to the guessability of password \cite{kelley2012guess}

\subsection{Method}

In the early state, password metering is used as a \ti{proactive password checker}, to prevent the user from using weak password \cite{bishop1990proactive, klein1990foiling}

Proactive password checker --> password strength meter

%
The password metering operates as the proactive password checker, which are based on the philosophy of \ti{Dictionary Attack}.

\cite{bishop1990proactive}  

\begin{table*}[ht]
	\centering
	\caption{The password guessing study \ti{Consider: Study, Method, Level/Metric, Data, Evaluation, Dataset, Result, Storage-space, complexity (time), character space}}
	\label{tab_pwd_meter_list}
	\def\arraystretch{1.2}
	\begin{tabular}{|c|c|c|c|} \hline
		 \ti{\tb{Study}}& \ti{\tb{Method}} & \ti{\tb{Level/Metric}} & \ti{\tb{Data}} \\ \hline
		%-----------------------------------------------------------------------------------------------------	
		
		Bishop \ea, 1990 \cite{bishop1990proactive}  & Rule-based, Dictionary & 2 & User infor, site infor, dictionary \\ %\cline{3-4}
		%
		
		Klein, 1990 \cite{klein1990foiling}  & Rule-based, Dictionary & 2 & User infor, dictionary \\ %\cline{3-4}
		%
		
		Spafford, 1992 \cite{spafford1992opus} & Bloom Filter ($\mathcal{O}(1)$ lookup dictionary) & 2 & Dictionary \\
		%
		
		Manber \ea, 1994 \cite{manber1994algorithm} & Improved Bloom Filter (approximately check (distance 1)) & 2 & Dictionary \\
		%
		
		Bergadano \ea, 1997 \cite{bergadano1997proactive} & Decision Tree (highly reduce the storage space ) & 2 & Dictionary \\
		%
		
		Bergadano \ea, 1998 \cite{bergadano1998high} & \ti{ProCheck} Decision Tree (improved from \cite{bergadano1997proactive}) & 2 & Dictionary \\
		%
		
		Yan, 2001 \cite{yan2001note} & Rule-based Entropy Measurement & 2 & $-$\\
		& (Applied for 7-digit password (only character and number)) &&\\
					
		
		Blundo \ea, 2002 \cite{blundo2002novel} & Perceptron (Neural network) & 2 & Dictionary \\
		
			
		Blundo \ea, 2004 \cite{blundo2004hyppocrates} & \ti{Hyppocrates} Decision Tree & 2 & \\			

		Ruffo \ea, 2005 \cite{ruffo2005enfilter} & EnFilter (based on ProCheck \cite{bergadano1998high}) & 2 & Dictionary (Italian, English \\
		 & & & Spanish and German) \\
		 
		Ciaramella \ea, 2006 \cite{ciaramella2006neural} & Multilayer Perceptron & 2 & Dictionary \& Generated strong password \\
				& \& Statistical techniques (improved from \cite{blundo2002novel})  && \\
		
		
		Burr \ea, 2006 \cite{burr2012electronic} & NIST entropy & & \\
		
		Jamuna \ea, 2009 \cite{jamuna2009novel} & Support Vector Machine & 5 & Very Weak, Weak, Good, Strong, Very Strong\\
		&&& Generated Dataset for Train/Evaluate \\

		Vijaya \ea, 2009 \cite{vijaya2009password} & Machine Learning (DT,SVM, MP, NB) & 5 & Generated password\\
		
		
		Suganya \ea, 2010 \cite{suganya2010proactive}& Dictionary \& SVM & 5 &	very weak, weak, good, \\
				&&& Strong, Very Strong \\
		
		
		Castelluccia \ea, 2012 \cite{castelluccia2012adaptive} & Markov \& Adaptive updating & bit length $\mathbb{R}$ & first state the definition of \quotes{ideal PSM}\\
		
		
		Houshmand \ea, 2012 \cite{houshmand2012building} & PCFG \& modify (1 edit-distance) to strengthen  & 2 & Real password \\
				& Dynamic update &&\\		
		
		Bonneau, 2012 \cite{bonneau2012statistical}&  Statistical Method & Bit length &  \\		
		
		Jakobsson \ea, 2013 \cite{jakobsson2013benefits}&  Password Parsing & Bit length & Build a parser to understand \\
				&&& password, then, classify \\
		
		Mazurek \ea, 2013 \cite{mazurek2013measuring}& existing methods &  & \\
		
		Dell \ea, 2015 \cite{dell2015monte} &monte carlo subsampling &bit length& dictionary\\
		
		Melicher \ea, 2016 \cite{melicher2016fast}&recurrent neural network&guess number &leaked password \{MG\}\\
		
		Wheeler \ea, 2016 \cite{wheeler2016zxcvbn} &heuristic, rule-based&guess number&password list/dictionary \{MG\}\\
		
		Wang \ea, 2016 \cite{wang2016fuzzypsm} &PCFG & &user's leaked passwords\{MG\} \\
		
		Xu \ea, 2017 \cite{xu2017password} &LSTM& leaked password&password\\
		
		Melicher \ea, 2017 \cite{melicher2017better} &RNN, Monte Carlo&real time feed back &password\{MG\}\\
		
		Ur \ea, 2017 \cite{ur2017design} &neural network, heuristics &feed back/suggested password&\\
											&&color-based strength&\\

		Galbally \ea, 2016 \cite{galbally2016new} & multi models &&real-valued score\\
		
		Guo \ea, 2018 \cite{guo2018lpse} &heuristic (cosine,edit) simi & 2 & client side\\
		
		Pal \ea, 2019 \cite{pal2019beyond} &GAN, word embedding&&password, modification path \{MG\}\\
		
		Liu \ea, 2019 \cite{liu2019reasoning} & Heuristic &guessing times&\\
		
		Dong \ea, 2021 \cite{dong2021rls} & LSTM, mangling rule&top percent& password, dictionary\\
																&& candidate password &mangling rule\\
		David \ea, 2021 \cite{david2021explainable} &rules, heuristics &&leaked password\\
		&&&mangling rules\\
		
		Hong \ea, 2021 \cite{hong2021enhanced} &rules&$[0, 9]$ &leaked password, korean keyboard \\
		
		
		\hline
	\end{tabular}
\end{table*}



The first paper

advantages and drawback of each approach

\cm{Provide password metering researches}

password strength is not a universal value, but depend on the context in which it is used \cite{galbally2016new}

Based on the operation mode, password metering could be divided in to client-side, and server-side.

could be classified into (\cite{galbally2016new})

\begin{itemize}
	\item Attack based methods:
		%
		\ti{1} unable to generalize well (\ie, a password will be scored with different strength under different attack methods).
		%
		\ti{2} require time to carry the attack, while user need the real-time score 
		
	\item Heuristic-based methods: LUDS (lower, upper, digital, symbol). Yet, raise some illogical results for some passwords.
	%
	Problem of this approach: assuming that all passwords are equally likely to be selected by humans.
	%
	This is effective against brute-force attack.
	
	\item Probabilistic-based methods:
	
	\item \textcolor{blue}{Machine learning?}
	
	\item Hybrid Approach \cite{galbally2016new}:
\end{itemize}

Describe the password metering's application/usecase. Give some of its example...


Then, explain its approaches...


Traditional method used entropy to measure the password strength.
%
Yet, this approach is accurate when the attackers randomly guess the password, which is not the case in practical situation.

So, tg

Avoid unrealistic assumptions which are in contrast to the user behavior.


There are two conceptual forms for password metering.
%

\tb{Statistical method:} \eg, Shannon entropy

\tb{Simulate adversarial guessing:} problem: time, resource \cite{melicher2016fast}
\subsection{Metric}
output of the meter: probability, likelihood, values in a specific rank, text (weak, strong...), reason/suggestion, guessing number/ time to guess

meter can be informative or enforcing \cite{golla2018accuracy}


several methods proposed metrics to evaluate the password strength

\subsection{Literature vs Commercial}

\section{Performance Evaluation}

\subsection{Dataset}
\subsection{Metric}


discuss year, size, languages...


==> reviewprocess.tex <==
\section{Review Process}\label{sec_review_process}

\cm{Present how to find the papers, method to conduct this research}
%

The keywords used in the searching process


